Payment Schemes from Limited Information with Applications in Distributed Computing

We propose a generic mechanism for incentivizing behavior in an arbitrary finite game using payments. Doing so is trivial if the mechanism is allowed to observe all actions taken in the game, as this allows it to simply punish those agents who deviate from the intended strategy. Instead, we consider an abstraction where the mechanism probabilistically infers information about what happened in the game. We show that payment schemes can be used to implement any set of utilities if and only if the mechanism can essentially infer completely what happened. We show that finding an optimal payment scheme for games of perfect information is \textsf{P}-complete, and conjecture it to be \textsf{PPAD}-hard for games of imperfect information. We prove a lower bound on the size of the payments, showing that the payments must be linear in the intended level of security. We demonstrate the applicability of our model to concrete problems in distributed computing, namely decentralized commerce and secure multiparty computation, for which the payments match the lower bound asymptotically.

==> 5_properties.tex <==
\subsection{Properties of Payment Schemes}
\label{properties}
We now present some additional properties that we may want our payment schemes to satisfy depending on the application. We show that the properties we state can be stated as linear constraints which fit nicely with the linear program constructed in the previous section. However, as the properties we state reduce the feasible region, likely they will increase the size of the maximum deposits. Whether a given property is worth this cost depends on the specific application in mind. Throughout this section, we consider some fixed finite game $G$ with information structure $\langle \Sigma, \P \rangle$, and let $\L$ be a payment scheme that implements a utility matrix $\E$.

\subsubsection{Honest invariance.} One possible issue with payment schemes is that they inherently change the game. In particular, a payment scheme may change the game even when all players are honest and play the intended strategy. This may dissuade the parties from playing the game to begin with, or may cause other adverse effects if some particular application requires the parties to receive a certain utility. The first property explicitly forbids this, by requiring that the utilities of the honest node remain unchanged. Formally, let $h$ be the index of the honest leaf, we say $\L$ is \emph{honest invariant} if $\U_{ih} = \E_{ih}$ for every $i = 1\ldots n$. We can easily implement this in our linear program by adding the following set of constraints:
\begin{align*}
	\sum_{k=1}\lambda_{ik}\P_{kh} = 0 && \forall\, i=1\ldots n
\end{align*}

\subsubsection{Zero inflation.} So far we have only required that the payment schemes do not inflate the currency by minting money. In general, we might want the payment scheme to `break even' in the sense that it also does not deflate the currency by locking away funds. To implement this we require that the sum of every column in $\L$ is exactly zero (or perhaps equal to the transaction fee on the blockchain). This has the effect that, for a given symbol, the sum of deposits for all players is zero. Formally, we say a payment scheme $\L$ has \emph{zero inflation} if $\mathbf{1}^\T\L = \mathbf{0}$. It is not hard to implement this as a linear constraint, simply change all inequalities of the form $\sum_{i=1}^n \lambda_{is+k} \geq 0$ to equalities.



\noindent In other words, we must be able to achieve game-theoretic security by giving utility from a party to another; it is not possible to e.g. simultaneously punish all parties for a specific action, and it is not possible to punish a party without rewarding another party. As such, the class of games that permit a zero inflation payment scheme have a specific structure, and we should not in general hope to achieve zero inflation.

Note that for certain `well-behaved' games, \cref{lemma:zero_inflation_U-E_column_sum_zero} also give sufficient conditions for zero inflation: namely, if there are fewer symbols than leafs and $\P$ is right-invertible then $\E$ has zero inflation if and only if the columns of $\U-\E$ sum to zero. This is an immediate consequence of the proof of \cref{lemma:zero_inflation_U-E_column_sum_zero} by following the deductions backwards.
